Mesh Watermark Removal Attack and Mitigation: A Novel Perspective of Function Space

Mesh watermark embeds secret messages in 3D meshes and decodes the message from watermarked meshes for ownership verification. Current watermarking methods directly hide secret messages in vertex and face sets of meshes. However, mesh is a discrete representation that uses vertex and face sets to describe a continuous signal, which can be discretized in other discrete representations with different vertex and face sets. This raises the question of whether the watermark can still be verified on the different discrete representations of the watermarked mesh. We conduct this research in an attack-then-defense manner by proposing a novel function space mesh watermark removal attack FuncEvade and then mitigating it through function space mesh watermarking FuncMark. In detail, FuncEvade generates a different discrete representation of a watermarked mesh by extracting it from the signed distance function of the watermarked mesh. We observe that the generated mesh can evade ALL previous watermarking methods. FuncMark mitigates FuncEvade by watermarking signed distance function through message-guided deformation. Such deformation can survive isosurfacing and thus be inherited by the extracted meshes for further watermark decoding. Extensive experiments demonstrate that FuncEvade achieves 100% evasion rate among all previous watermarking methods while achieving only 0.3% evasion rate on FuncMark. Besides, our FuncMark performs similarly on other metrics compared to state-of-the-art mesh watermarking methods.

==> chapter/checklist.tex <==
\section{Reproducibility Checklist}
This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
    \item Does this paper make theoretical contributions? (yes)
\end{itemize}
If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes)
    \item Proofs of all novel claims are included. (yes)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes)
    \item Appropriate citations to theoretical tools used are given. (yes)
    \item All theoretical claims are demonstrated empirically to hold. (yes)
    \item All experimental code used to eliminate or disprove claims is included. (yes)
    \item Does this paper rely on one or more datasets? (No)
\end{itemize}
If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)
    \item Does this paper include computational experiments? (yes)
\end{itemize}
If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes).
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
\end{itemize}

==> chapter/defence_bak.tex <==
\section{Function Space Watermarking}

\subsection{Methodology}


Our goal is to watermark both SDF and meshes extracted from them. In embedding phase, the owner embeds a binary message $\mathbf{M}\in\{0,1\}^{N_m}$ in SDF $F_\Theta$ to get the watermarked SDF $G_\Theta$. In the ownership verification phase, we expect the following application scenarios:
\begin{itemize}%[leftmargin=*]
    \item \textbf{Watermark decoding.} The investigator can decode the message from the given media to trace the leaker.
    \item \textbf{Watermark detection.} When the investigator cannot decode the complete message, he/she can still detect the watermark according to a statistical measure.
\end{itemize}
The media mentioned above can be either an SDF (white-box scenario) or a mesh extracted from an SDF (black-box scenario). In practice, we select SIREN \cite{siren} as our SDF backbone because our method requires accurate approximation on both $F(x)$ and $\nabla F(x)$.

To design a watermarking scheme satisfying both white-box and black-box scenarios, we embed binary messages $\mathbf{M}$ in the output of $F_\Theta$ through local deformations of implicit neural representations. In detail, we apply our watermarking embedding process as the following pipeline: (1) we first divide 3D space and SDF into $N_s*N_s$ partitions under the spherical coordinate system (Sec. \ref{sec: div}); (2) within each partition we embed one bit $b$, and we deform the partition according to $b$ (Sec. \ref{sec: embed}); (3) we design two measures for decoding process to verify the ownership for both white-box and black-box scenarios (Sec. \ref{sec: decode}).

\subsubsection{Spherical Partitioning} \label{sec: div}

Our first step is to divide 3D space under a spherical coordinate system since we only embed one bit in each partition. A spherical coordinate system is a coordinate system for three-dimensional space where the position of a given point in space is specified by three numbers $(r, \theta, \phi)$, where $r$ is the length of radial line connecting the point to the origin, $\theta\in [0, \pi]$ is measured by the angle between z-axis and the radial line, and $\phi\in[-\pi, \pi]$ is measured by the angle between x-axis and the orthogonal projection of the radial line onto the reference x-y plane.

A cartesian coordinate $(x,y,z)$ and spherical coordinate $(r,\theta, \phi)$ can be converted to each other by the following:
\begin{equation}
    \begin{split}
        \left \{
        \begin{aligned}
            &r=\sqrt{x^2+y^2+z^2}\\
            &\theta=\arccos(\frac{z}{r})\\
            &\phi=\arctan(\frac{y}{x})
        \end{aligned}
        \right .
        \quad
        \begin{split}
            \left \{
            \begin{aligned}
                &x=r\sin(\theta)\cos(\phi)\\
                &y=r\sin(\theta)\sin(\phi)\\
                &z=r\cos(\theta)
            \end{aligned}
            \right .
        \end{split}
    \end{split}
    \label{eq: cat_sph}
\end{equation}


We divide 3D space by equally dividing $\theta$ and $\phi$ into $N_s$ parts. In this case, the implicit neural representation is divided into $N_s*N_s$ parts. A spherical partition $\mathbf{\Omega}_{i,j}$ is a local region $\{(r,\theta,\phi)|\theta\in[\theta_i, \theta_{i+1}] \cap \phi\in[\phi_j, \phi_{j+1}]]\}$. Ideally, we expect the zero-isosurface to be evenly divided by each partition, so we normalize all meshes within a unit sphere before we build non-watermarked SDFs $F_\Theta$.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/defence/defence_pipeline.pdf}
    \caption{Watermark overview. We convert vertex coordinates into (a) a spherical coordinate system, which is further divided into $N_s*N_s$ partitions (denoted as $\Omega_{i,j}$). We further embed one bit in each (b) partition $\Omega_{i,j}$. The surface within $\Omega_{i,j}$ is deformed (c) outward if the embedded bit $b=1$, or else deformed (d) inward. The deformation strength is $10\times$ of the default setting.}
    \label{fig:defence_pipeline}
\end{figure*}

\subsubsection{Watermark Embedding} \label{sec: embed}
\textbf{Overview.} Our watermark is embedded by introducing independent deformations in each partition. To deform an SDF $F_\Theta$, we wrap the coordinate space of $F_\Theta$ using an analytic deformation function $D(\mathbf{y})$, which deforms a point $\mathbf{y}$ to $\mathbf{x}=D(\mathbf{y})$. Under this framework, the deformed SDF $G_\Theta$ can be represented as $G_\Theta(\mathbf{x})=F_\Theta(D^{-1}(\mathbf{x}))$ \cite{NFGP, deng2021deformed, liu2021editing}. We expect the following two properties: \textbf{(1)} $D$ is continuous and invertible so that $G_\Theta(\mathbf{x})$ can be calculated for $\mathbf{x}\in \mathbb{R}^3$; \textbf{(2)} $G_\Theta$ is still an \textit{sdf}, \ie, $G_\Theta$ and $\nabla G(\mathbf{x})$ are valid signed distance values and normal vectors, respectively, so that $G_\Theta$ can be still applied to downstream tasks. After achieving both properties, the final step is to remove the reliance of $D^{-1}(\mathbf{x})$ because malicious users can remove the watermark by removing $D^{-1}(\mathbf{x})$. We achieve this by distilling $F_\Theta(D^{-1}(\mathbf{x}))$ with a brand new SIREN network.
% \begin{itemize}
%     \item $D$ is continuous and invertible, so that $G_\Theta(\mathbf{x})$ can be calculated for $\mathbf{x}\in \mathbb{R}^3$.
%     \item $G_\Theta$ is still an \textit{sdf}, \ie, $G_\Theta$ and $\nabla_{x}G$ are \textit{sdf} fields and normal vector fields, respectively, so that $G_\Theta$ can be still applied to downstream tasks.
% \end{itemize}

\textbf{Define $D(\mathbf{y})$.} After dividing SDF into $N_s*N_s$ partitions along with the subdivision of 3D space in Sec. \ref{sec: div}, the next step is to make deformation within each partition to embed a binary bit. The deformation function $D(\mathbf{y})$ is defined within each region. Consider a partition embedded with a bit $b$, for all $\mathbf{y}\in\mathbf{\Omega}_{i,j}$,
\begin{equation}
    D(\mathbf{y})=
    \begin{cases}
        \mathbf{y}+\nabla F_\Theta(\mathbf{y})C(\mathbf{y})&b=1\\
        \mathbf{y}-\nabla F_\Theta(\mathbf{y})C(\mathbf{y})&b=0
    \end{cases}
    \label{eq: D}
\end{equation}
where $C:\mathbb{R}^3\mapsto\mathbb{R}$ is a scalar function ($C$ will be defined later). $D(\mathbf{y})$ moves $\mathbf{y}$ along the direction of surface normal $\nabla_{\mathbf{y}}F_\Theta$ with moving length $C(\mathbf{y})$ if $b=1$, otherwise moves $\mathbf{y}$ against the direction of surface normal. For convenience, we denote the operation that moves a point along the direction of its normal vector as \textbf{outward} and denote the operation that moves a point against the direction of its normal as \textbf{inward}. We show the visualized process in Fig. \ref{fig:embed} (b-c). We expect $C(\mathbf{y})$ to be smaller when $\mathbf{y}\in \mathbf{\Omega}_{i,j}$ is close to the edge of $\mathbf{\Omega}_{i,j}$. We achieve such feature by defining $C(\mathbf{y})$ as following:
\begin{equation}
    \begin{aligned}
        &C(\mathbf{y})=16\delta\frac{(\theta_{i+1}-\theta_{\mathbf{y}})(\theta_{\mathbf{y}}-\theta_{i})}{(\theta_{i+1}-\theta_{i})^2}\frac{(\phi_{j+1}-\phi_{\mathbf{y}})(\phi_{\mathbf{y}}-\phi_{j})}{(\phi_{j+1}-\phi_{j})^2}
    \end{aligned}
\end{equation}
where $\delta$ is a constant parameter representing the watermarking strengths.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,page=1]{figures/defence/embed.pdf}
    \caption{We show an SDF in (a). Within a partition embedded with bit $b$, we build one-to-one correspondence between original points $\mathbf{y}$ and watermarked points $\mathbf{x}$. (b-c) visualize the watermarking process when $b=1$, and (c) shows the watermarked SDF $G_\Theta$. In (d-e), we sample around zero-isosurface of $F_\Theta$, $G_\Theta$, respectively. In (e), the number of positive samples is significantly more than the number of negative ones, and thus, we reject the null hypothesis and detect the watermark.}
    \label{fig:embed}
\end{figure}


\textbf{Make $D$ invertible.} One way to make $D$ invertible is to approximate $D$ with invertible residual blocks \cite{NFGP}. However, in practice, we find the accuracy of invertible residual blocks cannot satisfy the accuracy requirements of watermarking. Besides, invertible residual blocks are ReLU-based networks, which make it hard to approximate both \textit{sdf} values and surface normals \cite{siren}.

\textbf{Newton's method calculates $D^{-1}(\mathbf{x})$.} $\mathbf{y}=D^{-1}(\mathbf{x})$ cannot be written in an analytic formula, since $\nabla F_\Theta(\mathbf{y})$ has no analytic formula. Fortunately, we can still derive $\mathbf{y}=D^{-1}(\mathbf{x})$ by calcuating the zero point of $\mathbf{y}\pm \nabla F_\Theta(\mathbf{y})C(y)-\mathbf{x}=0$. We apply Newton's method \cite{newtonmethod} to calculate the zero point as the following repeated process:
\begin{equation}
    \mathbf{y}_{n+1}=\mathbf{y}_{n}-\mathcal{J}^{-1}_{D}(\mathbf{y}_{n})\cdot D(\mathbf{y}_{n})
    \label{eq: newton_iteration}
\end{equation}
where $\mathbf{y}_{i}$ is the guessed zero point at $i$-th iteration, $\cdot$ is the matrix multiplication operation, and $\mathcal{J}^{-1}_{D}(\mathbf{y})$ is the inverse of Jacobian matrix of $D$ at the point $\mathbf{y}$. To calculate a correct zero point, this process is sensitive to the accuracy of $\mathcal{J}_{D}(\mathbf{y})$, which is derived from Hessian of the SDF: $\mathcal{H}_{F_\Theta}(\mathbf{y})$ (We show details in Supplementary Sec. A). However, $\nabla F_\Theta(\mathbf{y})$ is supervised with ground truth value only when $\mathbf{y}$ is on zero-isosurface. Thus, Newton's method may not find a zero point if the initialization $y_0$ is far from the zero-isosurface. To alleviate this issue, we randomly initialize multiple $y_0$ within $[-1,1]^3$. One hundred samples are enough to find the ground truth zero point.

\textbf{$\nabla G_\Theta(\mathbf{x})$ can be derived in an analytic way:} $\nabla G_\Theta(\mathbf{x})=\mathcal{J}_{D^{-1}}(\mathbf{x})\cdot \nabla F(\mathbf{y})$, where $\mathbf{y}=D^{-1}(\mathbf{x})$, and $\mathcal{J}_{D^{-1}}(\mathbf{x})$ can be derived directly from Eq. \ref{eq: D} (We show details in Supplementary Sec. A):
\begin{equation}
    \begin{gathered}
        \mathcal{J}_{D^{-1}}(\mathbf{x})=\Bigl(C(y)\mathcal{H}_{F_\Theta}(y)+\nabla C(y)(\nabla F_\Theta(y))^T+\mathcal{I}\Bigr)^{-1}\\
        \text{where} \ \ y=D^{-1}(x)
    \end{gathered}
    \label{eq: G_normal}
\end{equation}

\subsubsection{Ownership Verification} \label{sec: decode}
\textbf{Tagging points.} After dividing SDF into $N_s*N_s$ partitions, we decode each bit independently within each partition. As shown in Fig. \ref{fig:embed} (d-e), for all points $\mathbf{x}\in\mathbf{\Omega}_{i,j}$, we tag point $\mathbf{x}$ with bit 1 if $F_\Theta(\mathbf{x})>0$, otherwise we tag it with bit 0. Remember that we have white-box and black-box ownership declaration scenarios. In the black-box ownership declaration scenario, a mesh $\mathcal{M}$ is given to evaluate whether the mesh is generated from the watermarked SDF. In this case, we directly tag its vertex set $V$ with the binary bit. In the white-box ownership declaration scenario where an SDF is given, we can either extract a mesh from it through isosurfacing or sampling points on the zero-isosurface of the SDF. We use the same sampling strategy in \cite{NFGP} where they sample points from a rough shape and then apply Langevin dynamics to get an accurate sample on zero-isosurface. We denote $N_v$ as the number of vertices of the mesh or the number of sampled points on zero-isosurface.

\textbf{Measure.} Ideally, we expect all regions to have some points to decode the bit embedded in that region. However, when $N_s$ is large, and $N_v$ is small, no points may lie in a specific partition. In this case, that partition cannot be decoded. We design two measures for ownership verification: watermark decoding for dense points and watermark detection for sparse points.
\begin{itemize}%[leftmargin=*]
    \item \textbf{Watermark decoding.} A partition is tagged with bit $b$ if more than half of the points in that region are tagged with bit $b$. In this case, we can get a decoded message $\hat{\mathbf{M}}$, which can be compared with $\mathbf{M}$ with bit accuracy.
    \item \textbf{Watermark detection.} We say the point matches the partition it belongs to if the tagged bit matches the bit embedded in that region. In the case of sparse points, we detect the watermark by testing the following hypothesis \cite{LLM_WM}.
\end{itemize}
\begin{equation}
    \begin{aligned}
        H_0: \textit{the implicit neural fields/mesh is generated}& \\
        \textit{without knowledge of the secret message }\mathbf{M}.&\\
    \end{aligned}
    \label{eq: hypothesis}
\end{equation}
If the null hypothesis is true, the number of points that match their partition, denoted as $s$, has an expected value $N_v/2$ and variance $N_v/4$. The $z$-statistic for this test is
\begin{equation}
    z=2(s-N_v/2)/\sqrt{N_v}
    \label{eq: z_test}
\end{equation}
We reject the null hypothesis when $z$ is above a threshold given a significance level $\alpha$.

\textbf{How hard is it to remove the watermark?} We evaluate robustness against classic mesh attacks, including Gaussian noise, affine transformation, and remeshing. We find that Gaussian noise cannot remove our watermark unless the distortion made by Gaussian noise severely damages the visual effect. Affine transformation can remove the watermark easily because all points will be tagged by a wrong bit. To alleviate this issue, we align the given mesh (with vertex set $V$) with watermarked SDF $G_\Theta$ by minimizing:
\begin{equation}
    \begin{aligned}
        &(a^*,\beta^*,\theta^*,\phi^*,\mathbf{t}^*)=\\
        &\argmin_{a,\beta,\theta,\phi,\mathbf{t}}\sum_{v\in V} \lVert G_\Theta(a \mathbf{R}(\beta, \theta, \phi) v + \mathbf{t}) \rVert\\
    \end{aligned}
    \label{eq: align_mesh_SDF}
\end{equation}
where $a$ is the scaling factor, $\mathbf{R}(\beta, \theta, \phi)$ representing the function mapping a rotation angle $\beta$ and a rotation axis $(\theta, \phi)$ to the rotation matrix, and $\mathbf{t}$ is the translation vector. 3D rotation learning is hard due to the non-continuous mapping of $\mathbf{R}$ \cite{continuity_rotaion_learning}. Gradient descent can find the global optimum only if the initialized parameter set $(\alpha,\beta,\theta,\phi,\mathbf{t})$ is close to optimum $(\alpha^*,\beta^*,\theta^*,\phi^*,\mathbf{t}^*)$. We perform a coarse-to-fine-grained parameter search. For coarse-grained search, we use grid search to find a set of initialized parameter set $(\alpha,\beta,\theta,\phi,\mathbf{t})$. We use gradient descent within each grid for a fine-grained search to find the global optimum.


\subsection{Mitigation Evaluation}

% Given sdf/mesh, verify the msg accuracy ---> acc
% Given (sdf/mesh)+msg, verify the ownership or verify positive and false positive AUC ---> AUC
% By varying watermark strength, testing distortion and msg accuracy ---> acc & Chamber distance
% By varying message length ---> acc
% Given mesh, gauss/smoothing/ ---> acc
% Given sdf, varying marching cube ---> acc
% Given sdf, varying the resolution of meshes, verifying the acc & robustness


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth, page=1]{figures/experiment/visual.pdf}
        \caption{Visualize P2S}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth, page=2]{figures/experiment/visual.pdf}
        \caption{\textit{mesh-256} extracted from $F_\Theta$}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth, page=3]{figures/experiment/visual.pdf}
        \caption{\textit{mesh-256} extracted from $G_\Theta$}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth, page=4]{figures/experiment/visual.pdf}
        \caption{Visualize vertex tags $b$}
    \end{subfigure}
    \caption{(a-c) Visualize geometric differences between \textit{mesh-256} from $F_\Theta$ and $G_\Theta$. (d) Vertex tags $b$ on \textit{mesh-256} from $G_\Theta$.}
    \label{fig:visual_mesh}
\end{figure*}


% \begin{table*}
%     \centering
%     \small
%     \begin{tabular}{c| c| cccc| cccc| cccc}
%     % \toprule[1pt]
%     \multirow{2}{*}{Methods} & \multirow{2}{*}{Verify on} & \multicolumn{4}{c|}{8-bit} & \multicolumn{4}{c|}{16-bit} & \multicolumn{4}{c}{32-bit} \\\cline{3-14}
%     &  & CD$\downarrow$ & P2S$\downarrow$ & Normal$\downarrow$ & Acc$\uparrow$ & CD$\downarrow$ & P2S$\downarrow$ & Normal$\downarrow$ & Acc$\uparrow$ & CD$\downarrow$ & P2S$\downarrow$ & Normal$\downarrow$ & Acc$\uparrow$ \\
%     \hline\hline
%     \multirow{4}{*}{\textit{deform-mesh}}
%      & \textit{mesh-64} & 0.060 & 0.052 & 0.2014 & 73.00 & 0.058 & 0.047 & 0.1924 & 69.84 & 0.050 & 0.035 & 0.1824 & 67.61 \\
%      & \textit{mesh-128} & 0.051 & 0.049 & 0.1778 & 81.80 & 0.049 & 0.044 & 0.1728 & 85.56 & 0.043 & 0.031 & 0.1561 & 80.78 \\
%      & \textit{mesh-256} & 0.049 & 0.048 & 0.1723 & 89.88 & 0.047 & 0.043 & 0.1630 & 88.70 & 0.040 & 0.030 & 0.1488 & 89.21 \\
%      & $G_\Theta$ & / & 0.021 & / & 91.21 & / & 0.018 & / & 92.18 & / & 0.022 & / & 90.17 \\

%     \hline
%     \multirow{4}{*}{\tool}
%      & \textit{mesh-64} & 0.004 & 0.006 & 0.1065 & 82.90 & 0.004 & 0.006 & 0.1052 & 79.85 & 0.005 & 0.006 & 0.1125 & 75.75 \\
%      & \textit{mesh-128} & 0.003 & 0.004 & 0.0865 & 90.60 & 0.003 & 0.004 & 0.0871 & 87.56 & 0.003 & 0.005 & 0.0917 & 82.00 \\
%      & \textit{mesh-256} & \textbf{0.002} & 0.004 & \textbf{0.0828} & \textbf{95.69} & \textbf{0.003} & 0.004 & \textbf{0.0833} & 93.12 & \textbf{0.003} & 0.004 & \textbf{0.0889} & 94.37 \\
%      & $G_\Theta$ & / & \textbf{0.002} & / & 94.34 & / & \textbf{0.002} & / & \textbf{94.31} & / & \textbf{0.002} & / & \textbf{94.60} \\
    
     
%     \bottomrule[1pt]
%     \end{tabular}
%     \caption{Performance comparison with \textit{deform-mesh}. Note that ``/" means that CD and Normal differences cannot be used to measure the geometric distance between sampled points and a surface. This table shows that (1) \textit{deform-mesh} makes 9$\times$ more geometry differences than \tool, resulting in lower mesh quality; (2) decoding accuracy drops when isosurfacing resolution $r$ decreases; (3) message lengths have little effects on both geometry difference and decoding accuracy.}
%     \label{tab:baseline}
% \end{table*}

\begin{table*}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    % \toprule[1pt]
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Geometry Difference$\downarrow$} & \multicolumn{6}{c}{Accuracy \& Robustness$\uparrow$}\\\cline{2-9}
    & CD & Normal & w/o attack & Gaussian & Rotation & Translation & Remesh & Decimate \\
     \hline\hline
     Jiang \etal \cite{jiang2017reversible} & 0.009 & 0.0859 & 80.59 & 76.98 & 80.58 & 48.21 & 50.21 & 49.16\\
     Hiba \etal \cite{al2019graph} & 0.012 & 0.1195 & 87.48 & 54.31 & 50.40 & 50.41 &  52.35 & 51.50\\
     Tsai \etal \cite{tsai2020separable} & 0.085 & 0.2272 & 91.41 & 50.03 & 49.75 & 49.99 &  51.48 & 50.48\\
     Peng \etal \cite{peng2021general} & 0.009 & 0.0873 & 91.98 & 50.24 & 50.55 & 58.30 &  51.46 & 52.70\\
     % Peng \etal \cite{peng2022semi} & 0.008 & \textbf{0.0807} & 90.89 & \textbf{90.89} & 90.89 &  50.79 & 50.83\\
     \tool (Ours) & \textbf{0.002} & \textbf{0.0828} & \textbf{95.69} & \textbf{95.69} & \textbf{82.44} & \textbf{93.12} & \textbf{92.41} & \textbf{91.13}\\
    \bottomrule[1pt]
    \end{tabular}
    \caption{Performance comparison with traditional mesh watermarking methods, which watermark discretized meshes.}
    \label{tab:traditional}
\end{table*}

\begin{figure*}
  
  % \begin{minipage}[b]{0.60\linewidth}
  %   \centering
  %   \begin{tabular}{c| cccc |cccc}
  %   % \toprule[1pt]
  %    \multirow{2}{*}{sample $N_v$} & \multicolumn{4}{c|}{$\delta=0.0010$} & \multicolumn{4}{c}{$\delta=0.0005$} \\\cline{2-9}
  %     & FPR & TNR & TPR & FNR & FPR & TNR & TPR & FNR \\
  %    \hline\hline
  %    10 & 0.0 & 1.0 & 0.422 & 0.578 & 0.0 & 1.0 & 0.133 & 0.867 \\\hline
  %    50 & 0.0 & 1.0 & 0.977 & 0.023 & 0.0 & 1.0 & 0.656 & 0.344 \\\hline
  %    100 & 0.0 & 1.0 & 1.0 & 0.0 & 0.0 & 1.0 & 0.833 & 0.167 \\\hline
  %    1000 & 0.033 & 0.967 & 1.0 & 0.0 & 0.011 & 0.989 & 0.933 & 0.067 \\\hline
  %    5000 & 0.022 & 0.978 & 1.0 & 0.0 & 0.0 & 1.0 & 0.833 & 0.167 \\
  %    % 10000 & 0.056 & 0.944 & 1.0 & 0.0 & FPR & TNR & TPR & FNR \\\hline
  %   \bottomrule[1pt]
  %   \end{tabular}
  %   \captionof{table}{Empirical error rate for watermark detection under varied $N_v$.}
  %   \label{tab:auc}
  % \end{minipage}\hfill
  \begin{minipage}[b]{0.60\linewidth}
    \centering
    \begin{tabular}{c| ccc |ccc}
    % \toprule[1pt]
     \multirow{2}{*}{sampling $N_v$} & \multicolumn{3}{c|}{$\delta=0.0010$} & \multicolumn{3}{c}{$\delta=0.0005$} \\\cline{2-7}
      & precision & recall & F1 score & precision & recall & F1 score \\
     \hline\hline
     10 & 1.00 & 0.422 & 0.593 & 1.00 & 0.133 & 0.235 \\
     50 & 1.00 & 0.978 & 0.989 & 1.00 & 0.656 & 0.792 \\
     100 & 1.00 & 1.00 & 1.00 & 1.00 & 0.833 & 0.909 \\
     1000 & 0.968 & 1.00 & 0.984 & 0.988 & 0.933 & 0.960 \\
     5000 & 0.978 & 1.00 & 0.989 & 1.00 & 0.955 & 0.977 \\
    \bottomrule[1pt]
    \end{tabular}
    \captionof{table}{Error rate for watermark detection under varied $N_v$.}
    \label{tab:auc}
  \end{minipage}\hfill
  \begin{minipage}[b]{.35\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/experiment/z-score.pdf}
    \captionof{figure}{The average $z$-score as a function of the number of sampled points $N_v$.}% \caption{Figure caption}
    \label{fig:z-score-plot}
  \end{minipage}
\end{figure*}

\subsubsection{Setup}
We implement SIREN using four layers of MLPs with 256 channels to build both $F_\Theta$ and $G_\Theta$. Since we embed each spherical partition with one binary bit in the secret message $\mathbf{M}$, if the number of partitions $N_s*N_s$ is greater than the length of the message, we repeatedly embed messages until we consume all partitions. Unless explicitly mentioned, our experiment is conducted under the following settings. We set $N_s=32$ (\ie the spherical system is divided into $32*32$ partitions). The default embedded message has a 16-bit length. We select significance level $\alpha=0.001$. In this case, we reject the $H_0$ hypothesis when $z>3.09$ with a false positive probability of $10^{-3}$. We use marching cube \cite{lorensen1998MC} as our default isosurfacing method and the default watermarking strength $\delta=0.001$.

\textbf{Dataset.} To create a set of origin implicit neural fields, we use mesh fusion \cite{mesh_fusion} to create watertight meshes from ShapeNet \cite{shapenet2015} and Stanford Repo \cite{stanfordbunny}. All watertight meshes are normalized to the unit sphere. We further uniformly sample five million points on mesh surface where their \textit{sdf} values are zero and another five million points on $[-1, 1]^3$ where their sdf values are estimated following the same process in \cite{NFGP}. We then fit $F_\Theta$ \cite{siren} to the ground truth \textit{sdf}, and $\nabla F_\Theta$ to vertex normals.

\textbf{Baselines.} We first compare \tool with prior classic watermarking methods \cite{tsai2020separable,jiang2017reversible,al2019graph,peng2021general} which focused on discretized meshes. Since there is no function space mesh watermarking, we then design a rigorous baseline \textit{deform-mesh}, which makes deformations on a mesh instead of SDF: (1) perform spherical partitioning as is in Sec. \ref{sec: div}, (2) deform mesh vertices inward/outward with respect to the bit embedded in their belonging partitions, (3) fitting $G_\Theta$ from the watermarked meshes.

\textbf{Evaluation Methodology.} We verify the watermark on both watermarked SDF (white-box) and meshes extracted from it (black-box). A mesh extracted in resolution $r$ through isosurfacing methods will be denoted as \textit{mesh-$r$} for convenience. We aim to evaluate geometry differences (Chamfer distance, P2S distance, and Normal difference) and watermark accuracy ($z$-score and bit accuracy). Chamfer distance (CD) computes average bi-directional point-to-point distances, capturing large geometry differences but missing smaller geometric details. P2S distance computes the average point-to-surface distance from watermarked points to the original surface. Normal difference computes vertex normal difference between points and their nearest on-surface points, which captures differences for high-frequency geometric details when CD and P2S are small. CD and Normal differences are used to compute geometry differences between \textit{mesh-$r$} extracted from $F_\Theta$ and $G_\Theta$, while P2S is used to evaluate geometry distance between points and surfaces.

% \textbf{Default settings.} Unless explicitly mentioned, our experiment is conducted under the following settings. We set $N_s=32$ (\ie the spherical system is divided into $32*32$ partitions). The default embedded message has a 16-bit length. We select significance level $\alpha=0.001$. In this case, we reject the $H_0$ hypothesis when $z>3.09$ with a false positive probability of $10^{-3}$. We use marching cube \cite{lorensen1998MC} as our default isosurfacing method and the default watermarking strength $\delta=0.001$.

\subsubsection{Accuracy}


\begin{table}
    \centering
    \small
    \begin{tabular}{c|c| cccc}
    % \toprule[1pt]
     $\delta$ & Verify on & CD$\downarrow$ & P2S$\downarrow$ & Normal$\downarrow$ & Acc$\uparrow$\\
     \hline\hline
     \multirow{2}{*}{0.0005} & \textit{mesh-128} & \textbf{0.002} & 0.004 & \textbf{0.0744} & 71.85\\
      & $G_\Theta$ & / & \textbf{0.002} & / & 73.33\\
      \hline
     \multirow{2}{*}{0.0010} & \textit{mesh-128} & 0.003 & 0.004 & 0.871 & \textbf{87.56}\\
      & $G_\Theta$ & / & \textbf{0.002} & / & \textbf{94.31}\\
    \bottomrule[1pt]
    \end{tabular}
    \caption{Tradeoffs between geometry differences and watermarking accuracy by varying $\delta$. Note that ``/" means that CD and Normal differences cannot be used to measure the geometric distance between sampled points and a surface.}
    \label{tab:strength_acc}
\end{table}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/experiment/why_robust.pdf}
%     \caption{Robustness analysis under $\delta=0.001$. We show a local region within a partition embedded with $b=1$ (outward).}
%     \label{fig:why_robust}
% \end{figure*}


\textbf{Visual Quality.} We visualize meshes extracted from both $F_\Theta$ and $G_\Theta$ in Fig. \ref{fig:visual_mesh}, where we use point-to-surface (P2S) distance to evaluate geometry differences. Besides, we visualize vertex tags to understand better how secret messages are embedded.


\textbf{\tool vs. Baselines.} We conduct two independent experiments to compare the performance between function space watermarking (Tab. \ref{tab:baseline}), and the performance between \tool and discretized mesh watermarking (Tab. \ref{tab:traditional}). In the first experiment, we compare \textit{deform-mesh} and \tool under different message lengths in black/white-box scenarios. Under arbitrary verification media, Tab. \ref{tab:baseline} first shows that \textit{deform-mesh} has lower bit accuracy and makes 9$\times$ more geometry differences than \tool. The reason is that \textit{deform-mesh} embeds a watermark by first deforming meshes and then creating SDFs from watermarked meshes. Mesh deformation and SDF fitting errors make too many geometry differences, while \tool directly performs accurate deformation on SDFs with low geometry differences. In the second experiment, we compare \tool and discretized watermarking in Tab. \ref{tab:traditional}. Since prior works only focus on meshes, all evaluations of \tool are conducted on extracted \textit{mesh-256}. Tab. \ref{tab:traditional} shows that \tool outperforms prior methods and shows high robustness against remeshing and decimation attacks.


\textbf{Bit Accuracy in Watermark Decoding.} We evaluate bit accuracy under different resolution $r$ when only extracted \textit{mesh-$r$} are given (black-box) and different sampling number $N_v$ when $G_\Theta$ is given (white-box). In the white-box scenario, we directly sample $N_v=30000$ points on $G_\Theta$ and perform watermark decoding on sampled points. In the black-box scenario, we extract \textit{mesh-$r$} from $G_\Theta$ and perform watermark decoding on mesh vertices. \textit{mesh-64} has averaged $N_v=2764$ vertices and \textit{mesh-256} has averaged $N_v=48088$ vertices. Tab. \ref{tab:baseline} shows that we have $~94\%$ bit accuracy when $r=256$ while accuracy drops fast when points are sparser. This raises a question: can we still detect the watermark even if given vertices are extremely sparse?

\textbf{Error Rate in Watermark Detection.} We evaluate the error rate under different sampling numbers $N_v$. We use uniform sampling on the surface. We first show in Fig. \ref{fig:z-score-plot} that with the increase of $N_v$, $z$-score increases, and thus we have more confidence to reject $H_0$ to detect our watermark. Tab. \ref{tab:auc} shows that our watermark can be detected with only $N_v=50$ sampled points.

\textbf{Watermark Strength vs. Mesh Quality.} We conduct more experiments to evaluate the relationship between bit accuracy and mesh quality, the results of which are shown in Tab. \ref{tab:strength_acc}. By varying watermarking strength $\delta$, we achieve a good balance between mesh quality and bit accuracy when $\delta=0.001$.

\subsubsection{Robustness}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/experiment/gauss.pdf}
    \caption{Distorted \textit{mesh-128} after being extracted from $G_\Theta$.}
    \label{fig:visual_distortion}
\end{figure}
\begin{table}
    \centering
    \small
    \begin{tabular}{cc}
    \toprule[1pt]
     Isosurfacing & Acc\\\hline
     Marching Cubes \cite{lorensen1998MC} & 93.12\\
     Dual Contouring \cite{ju2002DC} & 87.75\\
     Neural Dual Contouring \cite{chen2022NDC} & 88.61\\
    \bottomrule[1pt]
    \end{tabular}
    \caption{Accuracy with different isosurfacing methods.}
    \label{tab:robustness_isosurface}
\end{table}




\textbf{Robustness on Isosurfacing.} The watermark on extracted meshes should be robust against different isosurfacing methods. In Tab. \ref{tab:robustness_isosurface}, we see our robustness against multiple isosurfacing methods \cite{lorensen1998MC, shen2021DMTet, nielson2004DMC, ju2002DC}.

\textbf{Robustness on Mesh Attack.} Combining Tab. \ref{tab:robustness} and Fig. \ref{fig:visual_distortion}, we evaluate robustness against distortions on Gaussian Noise, rotation, scaling, translation, simplification \cite{lindstrom1998edgecollapse}, Laplacian smoothing \cite{desbrun2023implicit}, quantization, and remeshing \cite{botsch2004remeshing}. Since Gaussian noise increases when the bounding box of meshes is smaller, we need to show the visual effect of arbitrary mesh attacks when the watermarked surfaces and extracted meshes are bounded by $[-1,1]^3$. In Fig. \ref{fig:visual_distortion}, Gaussian($\sigma=0.001,0.01$), Quantization(bit=8), simplification(90\%) and Smooth(iteration=3) make obvious visual distortions. We observe the high robustness in Tab. \ref{tab:robustness} that our watermark cannot be removed without obvious visual distortions. It is worth noting that our method is highly robust against remeshing, which is known as a common challenge in the mesh watermarking domain.

We provide further analysis of robustness. Arbitrary distortions increase the distance from watermarked vertices to $G_\Theta$. In Fig. \ref{fig:why_robust}(a), where no distortion has been made, extracted meshes only suffer from distortions caused by isosurfacing. In Fig. \ref{fig:why_robust}(b-c), remeshing inserts of points and edges, and decimation \cite{lindstrom1998edgecollapse} performs edge-collapse and points merging. In both cases, newly generated points maintain outward relative to the original surface.


\begin{table}
    \centering
    \small
    \begin{tabular}{cc}
    \toprule[1pt]
    Distortion & Acc\\
    \hline
    w/o distortion & 94.61 \\\hline
    
    Gaussian($\sigma=0.001$) & 94.61\\
    Gaussian($\sigma=0.005$) & 85.37\\
    Gaussian($\sigma=0.01$) & 64.87\\\hline
    
    Rotation($\pm \pi$) & 82.44\\
    Scaling($<25\%$) & 93.75\\
    Translation & 94.61\\
    Combined & 76.62\\\hline

    Simplication (30\%) & 93.75 \\
    Simplication (60\%) & 94.11 \\
    Simplication (90\%) & 76.37 \\\hline

    Smoothing (iteration=1) & 93.75\\
    Smoothing (iteration=2) & 93.12\\
    Smoothing (iteration=3) & 78.87\\\hline

    Quantization (bit=16) & 93.87\\
    Quantization (bit=12) & 91.01\\
    Quantization (bit=8) & 65.62\\\hline
    
    Remeshing & 93.46\\
    
    \bottomrule[1pt]
    \end{tabular}
    \caption{Bit accuracy with different distortion types.}
    \label{tab:robustness}
\end{table}



\section{Conclusion}


